Formalizing the Omega Test in Dafny

We present a formalization in Dafny of the Omega Test, an algorithm used to decide the satisfiability of a system of inequalities. The implementation defines executable representations for rational numbers, linear expressions, inequalities, equalities, divisibility constraints, and systems of constraints, together with their semantic interpretation through valuations. We fully specify and verify the implementation in Dafny. We describe the lessons learned and how the formalization process led to new insights into the algorithm.

==> eptcsdata.tex <==
\providecommand{\firstpage}{67}
\providecommand{\publicationstatus}{Mircea Marin, Adrian Cr\u{a}ciun (Eds.): FROM 2026\\
EPTCS 452, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.452.5}{10.4204/EPTCS.452.5}}
\pdfoutput=1

